MavVStream: Extending Database Capabilities for Situation Monitoring Using Extracted Video Contents

Query-based video situation detection (as opposed to manual or customized algorithms) is critical for diverse applications such as traffic monitoring, surveillance1 , and other types of environmental/infrastructure monitoring. Video contents are complex in terms of disparate object types and background information. Therefore, in addition to extracting complex contents using the latest vision technologies (including deep learning-based), their representation as well as querying pose different kinds of challenges. Once we have a representation to accommodate extracted contents, ad-hoc querying on that will need new operators, along with their semantics and algorithms for their efficient computation. Extending database framework (representation and real-time querying) for processing queries on video contents extracted only once is critical and this effort is an initial step in that direction. In this paper, we extend the traditional relation to R++ (vector attributes) and arrables to accommodate video contents and extend CQL (Continuous Query Language) with a few new operators to query situations on the extended representation. Backward compatibility, ease-of-use, new operators (including spatial and temporal), and algorithms for efficient execution are discussed in this paper. Classes of queries are identified based on their complexity to evaluate with respect to video content. A large number of small and large video datasets have been used (some from the literature) to show how our work can be used on available datasets. Correctness of queries with manual ground truth, efficient evaluation as well as robustness of algorithms is demonstrated. Our main contribution is couching a framework for a problem that is becoming very important as part of big data analytics based on a novel idea.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> texFiles/CQL-VAOperators.tex <==
\subsection{CQL-VA Operators}

% CQL with logical and physical windows has been extended with new operators that are needed for expressing situations in Set 1. Below, we define the operators, their semantics and complexity. We discuss their usage in section~\ref{sec:experiment}.

% \sharma{3/21}{for each operator, we need to give semantics, format, params and explain what it does Before going into its implementation! with space constraints, we may reduce implementation details!}

\subsubsection{StreamToArrable}

The StreamToArrable operator converts an R++ relation into an R++ arrable representation. This operator requires two arguments such as group by (gba) and assuming order (aoa). The gba attribute generates groups (similar to SQL group by) the tuples of the input relation and sorts them according to the aoa attribute specified. Each group is represented with a single tuple in the resulting table.

The semantics of the operator is following:

\noindent\texttt{StreamToArrable Str (gba, aoa)}

% where Str is the input stream, gba is a group by attribute (similar to SQL GROUP BY) and aoa is a unique assuming order (similar to SQL ORDER BY) attribute for converting into arrable representation. The aoa attribute should be order-able (either in ascending with ASC  or in descending with DESC). This operator can be applied when the specified gba and aoa attributes are not vectors themselves. The tuples in the Str relation is grouped using a hash table (using the gba attribute values as hash key) and the elements of each group is sorted according to the aoa attribute.  Finally, the tuples in each group are converted into arrable representation and populated in the output buffer for the next operator. 
In table~\ref{tab:ccrt-output}(b), the streamToArrable operator was applied on VS1 using gba as oid and aoa as fid. The resultant table contains two tuples since there are two different oids. 
 This operation can be applied with or without a window specification. Once the relation is in the arrable format, array-based computations can be applied to appropriate attributes.
StreamToArrable operator takes $\mathcal{O}(N + N \log N)$ time ( $N \log N$ for sorting) to convert an input relation of $N$ tuples into arrable representation. A single pass is made over each tuple for hashing. 
% Note that unlike a DBMS the stream tuples are in memory.

\subsubsection{Compress Consecutive Tuples (CCT)}
Since there exists a tuple for each element in the video stream, there is a lot of repetition of objects. It is not required to process each tuple for certain situations (e.g., counting number of objects). Additionally, the same object may appear multiple times in a video over a disjoint period. It is important to not lose this information present in the video (e.g., the same vehicle leaving and coming back multiple times.)

% As the same element (typically objects, but could also be others as well such as stationary objects) appears in multiple frames in a video (due to the pre-processing of each frame) and our representation is a tuple for each \textit{element in each frame}, there is likely to be a lot of repetition of objects that come in the way of efficient as well as the correctness of processing. Additionally, the same object may appear multiple times in a video over a disjoint period. It is important to not lose this information present in the video (e.g., the same vehicle leaving and coming back multiple times.)

The DISTINCT operator used for removing  \textit{multiple occurrences} cannot be used as our need is to remove \textit{consecutive multiple occurrences} and compress the current window (or relation) for further processing efficiently. For this, we introduce the unary operator Compress Consecutive Tuples (CCT) which will take an input relation (either R++ or R++ arrable) and reduce consecutive occurrences of specified attributes into one or two occurrences as indicated. The syntax of the operator is :
\hafsa{05/12/2022}{The CCT operator doesn't work without arrable.}

\noindent\texttt{CCT Str W(gba, aoa, option = \{\underline{first}|last|both\})}

where Str is the input relation, W is the window specification, gba is the group by attribute, aoa is the assuming order attribute, and the option parameter will retain the \textbf{first}, \textbf{last}, or \textbf{both} first and last occurrences (first being the default). The grouping and ordering process of this operator is same as StreamToArrable operator. After that, the first, last or both occurrence of tuples are extracted from each group (after grouping and ordering) according to the option specified. Lastly, a new schema definition is generated for the output relation.

An example of CCT operator on an input relation VS1 (shown in Table \ref{tab:camera-1}) is shown in Table~\ref{tab:ccrt-output}(c), where gba attribute is oid, aoa is fid and the option is specified as first. For ease of reading, some attributes are not shown in this table. Moreover we assume that the W attribute is specified as 5 ts rolling window with hop size 5.
\hafsa{05/13/2022}{Should we discuss about what rolling window is ?}
Furthermore, window 1 consists of frame number 1-5, window 2 from 6-10 and so on. If we use option both, we will get the result shown in Table~\ref{tab:ccrt-output}(d). This operator can be applied for any window specification or even without a window specification. However, if a window is specified, consecutive occurrences \textit{across windows} will not be considered consecutive as per its semantics. 
% This operator is idempotent. As MavVStream uses operator sequences, this operator is applied to the result of group by and ordering. 
%It is also possible to expand this operator into a sequence of three operators.


%asantra(3/8): CCRT changed to CCT in caption
\begin{table}[ht]
\centering
\caption { \textmd{Results of CCT Operator. Here object id is represented as oid, frame id as fid, The window W is defined as a 5 ts rolling window.}}
\subfloat[VS1]{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{[fid]} & \textbf{oid} & \textbf{BB} &  \textbf{[ts]} \\ \hline
1 		 & 1 	& [10,20,30,20]   & 1  \\ \hline
2 		 & 1 	& [11,20.5, 30,20]   & 2 \\ \hline
2       & 2 & [30,50, 8, 4]      & 2 \\ \hline
... 		 & ... & ...	   & ... \\ \hline
10       & 1  & [13,22,29,19]       & 10 \\ \hline
11       & 1  & [13,23,29,19]       & 11 \\ 
\hline
13       & 2  & [30,50, 8, 4]       & 13 \\\hline
\end{tabular}}
\qquad
\subfloat[streamToArrable VS1 (oid, fid)]{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{[fid]} & \textbf{oid} & \textbf{BB} &  \textbf{[ts]} \\ \hline
[1,2,...,11] 		 & 1 & [[],[],..,[],[]]	   & [1,2,...,10,11]  \\ \hline
[2,...,13] 		 & 2 & [[],...,[]]	   & [1,13]  \\ \hline
\end{tabular}}
\qquad
\subfloat[CCT VS1 W(oid, fid, first)]{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{\underline{fid}~~} & \underline{\textbf{oid}~~} & \textbf{BB} &  \textbf{ts~~} \\ \hline
1 		 & 1 & [10,20,30,20]	   & 1  \\ \hline
2 		 & 2 	   & [30,50,8,4]  & 2 \\ \hline
\end{tabular}}
\qquad
\subfloat[CCT VS1 W(oid, fid, both)]{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{\underline{fid}~~} & \underline{\textbf{oid}~~} & \textbf{BB} &  \textbf{ts~~} \\ \hline
[1,11] 		 & 1 & [[...],[13,23,29,19]]	   & [1,11]  \\ \hline
[2,13] 		 & 2 	   & [[30,50,8,4],[30,50,8,4]]  & [2,13] \\ \hline
\end{tabular}}
\label{tab:ccrt-output}
\qquad
\end{table}

We can apply other operators such as JOIN, SELECT  or AGGREGATE on the result set generated by CCT (shown in section~\ref{sec:experiment}). 
% For example, it can be used to find the duration of each occurrence of the object in the video or the number of frames in which an object appears in the video \textit{even when it occurs over disjoint intervals}.

The complexity of CCT operator is $\mathcal{O}(N)$ where $N$ is the number of tuples in each window. 

% The CCT operator performs a single pass over the current window after StreamToArrable operator is applied to the current window. Therefore, complexity of CCT operator is $\mathcal{O}(N)$ where $N$ is the number of tuples in each window.


% the number of tuples in the current input stream is $N$ and $G$ unique groups are generated after the grouping is performed on the specified gba attribute. After the ordering (requires $\mathcal{O}(N \log N)$ time) is performed, CCT extracts two tuples in the worst case (when option=both) is specified. In total, $2G$ tuples are fetched by CCT operator in the worst case. Therefore, the time complexity of CCT operator is $\mathcal{O}(N+N \log N+2G)$.

% The time complexity of CCT on an input stream Str is $\mathcal{O}(N+N \log N+2*G)$, where $N$ is the number of tuples in the current input buffer and $G$ is the number of unique groups generated after the GROUP BY operation (with specified gba attribute). Two tuples from each unique group is extracted after the ordering is done by the CCT. In total, 2*G tuples are extracted and converted to arrable representation. Hence, the complexity of CCT


% highest two elements from each group if the option is \textbf{both}. Hence, the CCT operator performs highest $2$ read operation for each group when both option is selected. Therefore, this has trivial effect on the complexity of this operator.

% Here $N$ is the number of tuples in the current input buffer, $G$ is the total number of groups for an unique gba vale, $t_i$ is the number of tuples in $i^{th}$ group of $G$). The initial scan and hashing of CCT operator requires $N$ reads. Since, hashing requires $\mathcal{O}(1)$ time, it is non trivial. Since the sorting operation for each group is performed individually, the complexity of sorting the elements of $i^{th}$ group is $\mathcal{O} (t_i \log t_i$). 
% \sharma{3/21}{no need to repeat if the complexity is same. just discuss differences. not sure what is 2*G operation. need to discuss!}


\subsubsection{Similarity Matching Operator: sMatch}
Since the appearance of object changes in each frame for a video, the feature vector generated for each object changes as well. As a result, two different feature vectors (same or different object) cannot be compared for equivalence using the logical (">", "<", "=") relational operators. We cannot answer the query Q1 in table~\ref{tab:QueryType} using oid since same object can be assigned different oid in the same video. Additionally, performing join over two windows also require for correctly answering queries.
The syntax of sMatch operator is following:

\noindent\texttt{sMatch (R1.attr, R2\.attr, metric, {threshold})}

where R1, R2 is the first and second window (or relation) that needs to be matched respectively. The attr parameter is typically a vector attribute (feature vector etc.) of the corresponding relation. 
We can specify a similarity metric using the metric parameter in sMatch. The similarity metric will compare two different feature vectors and generate a similarity value. Currently sMatch supports two different similarity metric such as cosine and euclidean distance. The threshold operator controls to what extent we can call two vectors similar. This operator returns a true value if the vectors match (matching similarity is above threshold) and returns false if they don't match. 


% We can specify a matching metric depending upon which type of VCE algorithm we are using. T


% The similarity of the input vector attributes
% is computed using a matching function. The matching function definition depends on the feature extraction algorithm used in pre-processing. This function generates a similarity value. The threshold operator controls to what extent we can call two vectors similar. This operator returns a true value if the vectors match (matching similarity is above threshold) and returns false if they don't match. 

% Since the pre-processing defines an object with feature vectors, the input to this operator is feature vectors for our case. Note that this is not limited to feature vectors and can be used on other attributes such as bounding boxes to infer whether an object has moved significantly or not. 


% This operator can be used in many ways. For example, if a video contains different object types (people, vehicles), it can be used to filter specific object types. It can also be used in a Join or cJoin operation to combine tuples with similar objects from two video streams or windows (e.g., entry and exit).

The complexity of this operator depends on the matching function used.

Therefore, we assume in this ~\pubtype, sMatch function takes a finite amount of time S to match two vectors. The time complexity of this operator is represented as $\mathcal{O}(S)$ in the rest of the paper. It is worth mentioning that, the cost of sMatch operator will be significantly higher than operators like "=","<", ">" of SQL.

\hafsa{05/13}{May be the complexity of euclidean and cosine distance should go there}

\subsubsection{Consecutive Join (cJoin) Operator} 
Join in relational model performed using logical operators. Since, these operators are not applicable for attributes such as feature vectors. Joining of two video streams (or windows) can be performed employing sMatch in the join condition. As mentioned earlier, the repetition of frames across a video (or window), makes a join operation very inefficient. We need to be able to compare and match the same object (feature vectors) once and disregard other \textit{consecutive} occurrences. cJoin is defined on two R++ arrable streams (or windows), where the join condition should include sMatch if the feature vectors are compared. The syntax of this operator is 
\begin{verbatim}
R1{w_1, gba_1, aoa_1} cJoin(join-condition) 
         R2{w_2, gba_2, aoa_2}
\end{verbatim}
where R1 and R2 are two input relations of R++ type, $w_1$ and $w_2$ are the window specification. For each relation the gba and aoa attributes need to specified. The join operation discards consecutive occurrence of matched tuples in the two input windows after grouping and ordering using StreamToArrable operator.

%DEBS Description-------------------
% A join operation in the relational model is computed based on exact matches of the attributes. As mentioned earlier, an exact match of two objects cannot be performed because their feature vectors are not identical across occurrences. Hence, the sMatch operator described above is used in the join condition of the cJoin operator proposed in this paper. 

% Consecutive join or cJoin, is a join suited for merging two relations using the sMatch function. The traditional join is defined in terms of the cartesian product followed by selection (although not implemented in that fashion). This kind of join on video data is not only extremely inefficient (due to the cost of sMatch) but also produces enormous results that are not useful. We need to be able to compare and match the same object once and disregard other \textit{consecutive} occurrences. Consecutive Join (or cJoin) is defined on two streams (with or without window specification) and a join condition is provided. Typically, this join condition would include the sMatch operator, as part of its condition, on feature vectors. This operator also needs the attributes gba and aoa described as part of the CCT operator. The syntax of this operator is
% \begin{verbatim}
% R1{w_1, gba_1, aoa_1} cJoin(join-condition) 
%          R2{w_2, gba_2, aoa_2}
% \end{verbatim}
% where Stream1 and Stream2 are two input streams to join, $w_1$ and $w_2$ are the window specification of these streams respectively. The cJoin operator joins the tuples of two stream windows in the current input buffer. The join operation discards consecutive occurrence of matched tuples in the two input windows after grouping and ordering using StreamToArrable operator. The cJoin can also be applied without the use of the sMatch as part of the join condition (when we don't need to match objects). The semantics remains the same and gba and aoa specifications are needed.

% The cJoin operator groups and sorts the input in a similar way as CCT and StreamToArrable.  The joining operation is performed by matching the tuples from each group in Stream1 with all the tuples of each group in Stream2. Consecutive occurrences of the matched tuples from each group in each relation are discarded. If no match occurs between two video streams, then no output is produced. 

Although it is possible to use the CCT operator in default mode to filter multiple consecutive occurrences from each window of a stream and then apply the traditional join, there is a subtle difference between the two ways of computing. cJoin is likely to be more accurate when joining two streams where a similarity match is required. The cJoin allows multiple comparisons of an attribute in the same equivalence class (i.e., having the same oid) with multiple tuples of the other window (Stream2) in the same equivalence class (i.e., same oid in that stream) and still avoid the cartesian product as soon as a match is found. This is likely to produce better and more accurate results because similarity comparisons are inherently approximate. One can view the join on CCT filtered streams as a faster and approximate version of cJoin. However, both can correctly deal with temporally disjoint appearances of objects. Even for window-based cJoin where the window may be large, it is possible to apply the CCT operator on each window to reduce their size and then apply cJoin along with the sMatch operator. Although this may result in missing some matches, the size of the synopses to be maintained will be significantly smaller. 

It is not possible to compute the cJoin operator using a hash-based approach (because it needs sMatch to measure two objects equivalence). The cJoin operator is implemented using the nested loop join (supported by MavVStream architecture). For two input windows with $N_1$ and $N_2$ tuples, the worst case complexity of cJoin operator will be $\mathcal{O}(N_1N_2S)$, where S is the time complexity for sMatch operator.
On the other hand, if we apply the CCT operator before joining, the complexity will reduce significantly.
Lets assume the number of tuples in both windows is $G_1$ and $G_2$. Therefore, the complexity of cJoin will be $\mathcal{O}(G_1G_2S)$. Note that the size of $G_1$ and $G_2$ will be significantly smaller than $N_1$ and $N_2$ (the CCT operator extracts highest two tuples from each group). As a result, the run time complexity of cJoin will reduce significantly. This is important, when we are joining two large windows and a large number of objects need to be matched.

\hafsa{05/13}{Need to check if logical operator is supported under cjoin. Also check if join can be done after arrable}


\subsubsection{Direction}
Direction is a temporal operator in CQL-VA for inferring direction of objects in a particular window. This operator is useful for composing higher level events (e.g., identifying trajectory of an object or group of objects). The syntax of the operator is following:
\begin{verbatim}
Direction(R1, R1.attr) 
\end{verbatim}
where R1 is a R++ arrable relation and attr is an attribute of type bounding box. Lets assume, the first and last bounding box of an object in a window is 
$bb_1 (x1, y1, w1, h1)$ and $bb_2(x2, y2, w2, h2)$, where $x_i$ and $y_i$ are the bottom left corner point, $w_i$ and $h_i$ are width and height respectively. A direction type $D_t \in {North, South, East, West, North East, North West, South East, South West}$ is assigned to that particular object.

A set of rules are associated with this operator to compute the eight directions. The rules are given below:
\begin{verbatim}
((y2-y1)>0 and (x2-x1)=0) => D_t = NORTH
((y2-y1)<0 and (x2-x1)=0) => D_t = SOUTH
...
\end{verbatim}

% ((y2-y1)=0 and (x2-x1)>0) => D_t = EAST
% ((y2-y1)=0 and (x2-x1)<0) => D_t = WEST
% ((y2-y1)>0 and (x2-x1)>0) => D_t = NORTH EAST
% ((y2-y1)>0 and (x2-x1)<0) => D_t = NORTH WEST
% ((y2-y1)>0 and (x2-x1)=0) => D_t = SOUTH EAST
% ((y2-y1)<0 and (x2-x1)<0) => D_t = SOUTH WEST

The result of this operator adds an enumerated type attribute DIRECTION (similar to aggregate functions) and outputs a tuple with an additional attribute whose value is one of eight directions. Note that this is the net direction of motion and not the trajectory. 


% --------Debs Description
% This is an example of how stream processing can be used to infer direction of object movement which can be used an event for composing higher level events, such as u-turn. 
% This operator is applied over the result of the CCT operator for efficiency with \textit{both}specified as the parameter.  The semantics of this operator is :

% \begin{verbatim}
% Direction(Stream1, dir.attr) 
% \end{verbatim}
% where dir.attr is an attribute of the input relation Stream1. The current implementation of Direction operator takes only bounding box as a dir.attr value to identify the direction of movement. Lets assume, the bounding boxes of object id $i$ is $bb_1 (x1, y1, w1, h1)$ and $bb_2(x2, y2, w2, h2)$ for the first and last occurrence after applying CCT. Using the $x$ and $y$ coordinates of the bounding boxes, a direction type $D_t$ is assigned to that particular object. A set of rules are associated with this operator to compute the eight directions. The rules are given below:
% \begin{verbatim}
% ((y2-y1)>0 and (x2-x1)=0) => D_t = NORTH
% ((y2-y1)<0 and (x2-x1)=0) => D_t = SOUTH
% ((y2-y1)=0 and (x2-x1)>0) => D_t = EAST
% ((y2-y1)=0 and (x2-x1)<0) => D_t = WEST
% ((y2-y1)>0 and (x2-x1)>0) => D_t = NORTH EAST
% ((y2-y1)>0 and (x2-x1)<0) => D_t = NORTH WEST
% ((y2-y1)>0 and (x2-x1)=0) => D_t = SOUTH EAST
% ((y2-y1)<0 and (x2-x1)<0) => D_t = SOUTH WEST
% \end{verbatim}
% The result of this operator adds an enumerated type attribute DIRECTION (similar to aggregate functions) and outputs a tuple with an additional attribute whose value is one of eight directions. Note that this is the net direction of motion and not the trajectory. 


% As a result, each tuple will have an attribute (in our case bounding box) which is a vector of two elements. They will be the bounding boxes of the first and the last consecutive frames of an object. This operator essentially computes the direction of motion using the dir attr as one of the eight directions using the two bounding box values. 


% --------DEBS CEP
% The DIRECTION operator can be incorporated with the event generator operator to detect a composite event. In our example,  the event "moving north" is generated if the value of the attribute is "north". Similarly, events "moving left", "moving south" is generated. The event detector uses this event stream to detect composite events which are specified separately and rules can be associated with any composite event.

==> texFiles/MavStream_Implementation.tex <==
%%\newpage

%\begin{wrapfigure}

%\end{wrapfigure}

\section{MavVStream Architecture}
\label{sec:macvstream-implementation}
The MavVStream (\textbf{Mav}erick \textbf{V}ideo \textbf{Stream} Processing System) shown in Figure~\ref{fig:mavvstream} augments a traditional stream and event processing system. MavVStream is a client-server-based architecture where a query is processed in a continuous manner (known as Continuous Query or CQ) when submitted by a client. 

An input CQ in the form of an operator computation sequence is converted into a query plan object by the input processor module of the client-side (in Figure~\ref{fig:mavvstream}). The query plan object contains all the necessary information for processing that CQ. This plan object is instantiated by the instantiator module which creates an executable CQ tree by instantiating each operator along with input and output buffers needed for processing that operator. A scheduler is also associated with each operator for scheduling it using supported scheduling strategies. 

When a query is activated for execution, the feeder populates the input queues to the server and the scheduler starts scheduling the CQ operators. The input queue contains the pre-processed relational representation of the input video streams.

The integrated underlying base of the MavVStream architecture supports all the Relational operators including SQL-92 aggregation operators. Additionally, new operators and data model extensions proposed in this paper are incorporated in the server side to express and compute the outputs of the continuous queries. The multi-threaded feeder reads the relational representation (written as serialized objects at the time of pre-processing) of the pre-processed video contents. Additionally, it feeds them into the input buffers of leaf operators at individually specified rates. The server process the CQ's using the currently available pre-processed data and generates interesting events or results of CQs.

The long-term goal for this system is to incorporate more operators, optimization of added operators along with the old ones,  support Quality of Service (QoS) requirements (by adding relevant scheduling and load shedding strategies) to progress towards a real-time system for situation monitoring. We expect this to be part of a larger situation analysis system that includes disparate data types for fusion applications. 


\begin{comment}
The main modules of MavVStream are :
\begin{enumerate}
\item \textbf{User Input (Client):} A client program is used to specify a continuous query request.  This request specifies which data sources to use and the structured query to apply to those sources. The request also specifies the start and end time of the query, the scheduling strategy and other user-definable configurations for the query.
\item \textbf{Input Processor:} The input processor component of the MavVStream server is responsible for listening to query requests and converting them from the incoming XML to query plan objects.  Query plan objects contain the information needed to setup and run a query, including a reference to the final (or root) operator of the query.
\item \textbf{Instantiator:}  The instantiator initializes and instantiates every operator in the query plan object. It sets the input and the output buffers for each operator for the tuples. The instantiator gets all the  information about the operator from operator node data and initializes them. It also associates the scheduler with the operator but does not start them.
\item \textbf{Scheduler:} The scheduler takes care of scheduling the operators. It is not done at the tuple level since the number of tuples to be handled by the system is enormous. The ready queue is maintained by the scheduler which decides the order in which the operators have to be scheduled.
\item \textbf{Feeder:}  The feeder feeds the stream data to the leaf operators. The feeder thread reads the tuples from the disk and feeds to the input buffer of the leaf operators. The data rate to feed tuples to the feeder is separately specified as a user input.
\item \textbf{Run Time Optimizer:}  Run time optimizer is implemented to improve quality of service (QOS). It aims at maximizing the output rate of query evaluation plans.
\end{enumerate}


MavVStream is beeing implemented with an object-oriented approach using the Java programming language.  All files are maintained in the package - edu.uta.dsms.  Its sub-package structure is as follows:

\begin{enumerate}
\item \textbf{dsms.core:} This package contains classes necessary for defining streams and queries. It also contains classes that provide support for Boolean logic expressions and their evaluators.  This package is referenced by both client and server programs.
\item \textbf{dsms.server:} It contains classes for all server operations including classes that implement the MavVStream architecture.  It also also contains a helper class that de-serializes XML-based query specifications received by the server (XML over TCP).
\item \textbf{dsms.client:} It contains classes for a remote client, for constructing queries and transmitting them via XML over TCP to the server.
\end{enumerate}

The MavVStream system has been extended from MavEStream System to process queries on preprocessed input video data and currently supports operators to handle queries based on bounding boxes and feature vectors. We are currently using input/output buffers as abstract classes and interfaces as each operator inside the query needs to have a distinct buffer of its own to process a video stream. We also have abstract classes for operator node data, so that each operator can setup its own data when it runs.
\end{comment}






==> texFiles/data-model-for-video-contents.tex <==
\begin{comment}
\subsection{Data Model for  Video Contents}
\label{sec:data-model}
For satisfying first normal form  (or atomic attributes), attributes having multiple values such as bounding boxes have to be represented using multiple attributes in a traditional relational representation. For example, a bounding box of an object has 4 values corresponding to the base coordinates along the x and y-axis of the frame \& width and height of the box. Representing a bounding box using relational data model will require four attributes. In addition, video pre-processing can generate variable length object definitions, such as feature vectors. Moreover, the data type of these definitions are vectors, multi-dimensional matrix etc. Representing these data types with the relational model is not possible. For example, deep learning-based object detection methods generate 2-D matrices as feature vectors. A feature vector with $10 \times 10$ matrix dimension would require $100$ attributes in relational model representation  (practically feature vectors have larger dimension).

Another drawback of the Relational data model is its inherent row-oriented computation; if one wants to compare elements from two rows, a join is needed to bring them into a single row.
Furthermore, the lack of ordering for performing computations  (as it is a set-based model) does not suit video data that is inherently a sequence of frames  (and time stamps). All of the above are issues that need to be overcome for video content analysis. 

Ordering is important to make sure frames are not processed in arbitrary order, and sequences  (of bounding boxes, frames, etc.) are used correctly for computing various actions. If one wants to compute the number of frames  (or duration) in which the same object appears  (or duration of an object in the video), one needs to bring together consecutive frames for performing computations. %%Otherwise, large numbers of joins need to be performed.

Hence, as a minimum, a vector or array data type  (whose contents may themselves be vectors/arrays) needs to be added to the data model. Besides, we need enumerated data types to capture, for example, the direction of motion in one of the 8 directions  (North, Southwest, etc.). It should also be possible to order the contents of these vectors on one or more attributes of interest. 

An extension to the relational model that has been proposed to deal with ordered computations  (useful in the financial domain for computing moving averages and other domains) is an \textbf{arrable}~\cite{lerner2003aquery}. The arrable allows representing a relational value with attributes that can have an array of scalar values  (or vectors). The relational operations of SQL  (e.g., \texttt{SELECT, PROJECT, JOIN}) are backward compatible with an arrable. The attributes of a relational representation can be grouped and ordered into a single attribute using the group by and assuming order functionality of arrable.



\end{comment}





==> texFiles/data-representation.tex <==
%%\newpage




\begin{comment}
\subsection{Limitations of SQL OVER Clause}
\label{sec:windows}
The join operators in SQL can become blocking operators as they require all the input relations present in memory before computation. It is not possible to read all the stream data at once due to its unbounded nature. Therefore, the notion of windows  (both physical and logical~\cite{Babcock:PODS02:Models, DBLP:journals/vldb/ArasuBW06}, predicate-based windows~\cite{DBLP:journals/sigmod/GhanemAE06}) have been introduced to circumvent the blocking operators by stream processing frameworks and in CQL. 

The OVER clause was introduced into SQL 2003 for supporting queries with window- and order-based computation. Briefly, the OVER clause can be used in a SELECT clause to aggregate using a window specification. A window function in SQL performs a calculation across a set of table rows that are somehow related to the current row. This is comparable to the type of calculation that can be done with an aggregate function. But unlike regular aggregate functions, the use of a window function does not cause rows to become grouped into a single output row - the rows retain their separate identities. You can also control the order in which rows are processed by window functions using ORDER BY within OVER\footnote{Please refer to ~\url{https://community.modeanalytics.com/sql/tutorial/sql-window-functions/} for a tutorial on SQL 2003 and OVER clause.}. 

A restriction of the OVER clause is that it cannot be used with a GROUP BY clause. Also, joins are not possible over frames. Multiple tables can be used in the FROM clause as the OVER clause is applied to the result of the WHERE clause  (i.e., theoretically, after the Cartesian product and restriction by the WHERE clause.) Below we use the SQL  (with OVER clause) in Oracle  (version 10.2.0.4.0) to express some of the queries in \textbf{set 1} in section~\ref{sec:query-classes} to represent the lacking of OVER clause in details.

Consider the schema shown below for \textit{camera 1} where [attribute] represents a vector data type. Note that feature vectors are a vector of vectors. Table~\ref{tab:camera-1} shows a sample of the extracted data represented as a relation using vectors. For brevity, assume that object 1 occurs in consecutive frame numbers 1 to 30, object 2 in 1 to 20, and reappears from 31 to 61. Also assume that object 3 appears in consecutive frames from 41 to 61. It is worth mentioning that, in reality the feature vectors and bounding boxes dont hold value like "fv1-1" and "bb1-1". Since, this is an imitation of real-life representation and we have space constraints, these values are used alternatively.

\noindent VS1  (Camera\_id ~as~ cid,  Frame\# ~as~ \underline{Fr\#},    Object\_id ~as~ \underline{oid},   \\
Feature\_Vector ~as ~[FV], Bounding\_box ~as ~[BB], Timestamp ~as ~ts)

%%\begin{wraptable}{r}{0.6\textwidth}
\begin{table}[ht]
\caption { \textmd{VS1: Entry Video Stream as a Relation with Vector Attributes}}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{cid} &\textbf{\underline{Fr\#}} & \underline{\textbf{oid}} & \textbf{[FV]} & \textbf{[BB]} 		& \textbf{ts} \\ \hline
1 		   & 1 		 & 1 	   & [fv-1] & [bb1-1] & 1  \\ \hline
1 		   & 1 		 & 2 	   & [fv2-1] & [bb2-1] 	& 1  \\ \hline
1 		   & ... 	 & ...	   & ...  & ... 	& ...  \\ \hline
1 		   & 20 	 & 2 	   & [fv2-20]  & [bb2-20] 	& 15  \\ \hline
1 		   & 30 	 & 1 	   & [fv1-30]  & [bb1-30] 	& 21  \\ \hline
1 		   & ... 	 & ...	   & ...  & ... 	& ...  \\ \hline
\end{tabular}
\label{tab:camera-1}
\vspace{-5pt}
\end{table}

The query "How many people entered the building every hour on the hour?" cannot be expressed as there is no time-based window supported in the OVER clause. It is not possible to convert this query into a tuple-based window query as the number of occurrences of objects in a frame  (or consecutive frames) is not known. However, the other query "How many people entered the building between a given interval  (say 21 and 41 inclusive) can be expressed without using the OVER clause as:

\begin{verbatim}
SELECT MIN (ts), MAX (ts), 
COUNT (DISTINCT oid)
FROM   VS1 WHERE  ts >= 21 AND ts <= 41;
\end{verbatim}

The above query is not suitable for video situation analysis as multiple, temporally disjoint appearances  (an object can enter multiple times) of the \textit{same} object need to be identified as separate occurrences. Currently, this is not possible. For example, object 1 is counted once although enters twice in that interval.

Similarly, the query "Identify the slowest/busiest hour of the day  (with respect to the number of people entering)" cannot be expressed as it needs the query mentioned above and choose the hour with the minimum or the maximum number of people\footnote{If a single camera is recording both entry and exit, it is necessary, as part of pre-processing, to identify objects as entering or exiting using an enumerated-type of the attribute. In that case, a single relation can be used and by partitioning the relation on that attribute, this query can be expressed.}.

Although it is possible to join two computed relations each using window operators in SQL, to the best of our knowledge, it is not possible to perform joins on window frames generated for each relation  (as only one can be used along with the OVER clause. This query, ideally, needs to check  (match or join) each object entering  (with a timestamp ts1) with all objects exiting with timestamp ts to ts+1hr as a window frame. This window frame cannot be specified using another relation window frame.

An alternative is to cast this query in a different way. One can do a regular join and \textit{then} check whether the time intervals were within the range expected. The following query does that.

\begin{verbatim}
SELECT VSE.ts as e_time, VSX.ts as x_time, 
          VSE.Obj_id
FROM VS_entry VSE, VS_exit as VSX
WHERE sMatch (VSE.FV, VSX.FV, threshold) AND 
          VSX.ts <= VSE.ts + 1 hr ;
\end{verbatim}

In the above, the sMatch function is used for comparing feature vectors to determine whether they match based on whether the similarity value between the two feature vectors is greater than equal to the threshold specified  (see more details on section \ref{sec:cql-vaimplementation}). As it is easy to notice, this has two problems: i) the entire video is needed as input and ii) the above will perform join on \textit{all pairs of tuples}  (actually a Cartesian product) which is overkill. This will not be meaningful for large videos or when the monitoring is continuous. Queries in Set 2 cannot be expressed at all as they require extraction and representation of actions  (e.g., turning around) which is currently lacking.

Based on our attempt to express meaningful video situations, we have identified the following limitations of SQL even with the availability of the OVER clause:
\begin{packed_itemize}
\item OVER does not support time-based windows.
\item OVER Frame specifications cannot move the upper and lower bounds arbitrarily.
\item Although multiple OVER clauses can be specified on \textit{different relations}, windowing clause is applied to the result of the FROM and WHERE clause, not for each relation\textit{before} joining and applying the WHERE clause.
\item Window-based joins are not allowed under the current specification of the OVER clause.
\item Window offsets between joins cannot be specified currently.
\end{packed_itemize}

The limitations of OVER clause can be overcome by using AQuery~\cite{lerner2003aquery}  (an extension of SQL). 
Using AQuery, we can rewrite the above query to select objects that occur in n consecutive frames. 

$\vspace{10pt}$
\begin{verbatim}
SELECT          [Fr#], oid, [FV], [BB], [ts]
FROM            VS1
ASSUMING ORDER  Fr#
WHERE           consecutive (40, [Fr#])
GROUP BY        oid
ORDER BY        vs1.oid ASC
\end{verbatim}


For n as 40, the above AQuery results in the output shown in Table~\ref{tab:arrable}. We do not include cid and [BB] in the result to save space. Since, n is set as 40 it doesn't take into account the frames from 1 to 40.
%%\begin{wraptable}{r}{0.6\textwidth}
\begin{table}[ht]
\caption {\textmd{Result of AQuery on VS1 in Arrable Representation}}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{ \underline{Fr\#}} & \textbf{oid} & \textbf{[FV]} & \textbf{[ts]} \\ \hline
[41, ..., 71] 		 & 2 	   & [fv2-41, ..., fv2-71] & [22, 42]   \\ \hline
[41, ..., 71] 	 & 3	   & [f4-31, ..., fv4-71]      & [22, 42]  \\ \hline
\end{tabular}
\label{tab:arrable}
\vspace{-25pt}
\end{table}
%

Ordering and grouping can be done on any attribute(s) to get the values of vectors as a sequence using AQuery. Various vector-based computations can be performed on them without resorting to multiple joins, making the query easy to understand and optimize. Therefore, counting the number of people within each hour on Table~\ref{tab:arrable} is easier than using the OVER clause.

However, this by itself is not sufficient for expressing meaningful situations in videos. For example, in the above, unless the consecutive occurrences are satisfied for a given value, we cannot assume fixed size computations that may be meaningful in other domains (e.g., financial applications) for computing moving averages, etc. For the video domain, the number of frames  (or duration) in which an object appears is not known in advance. 
% One option is to try and use the current notions of windows (discussed in section~\ref{sec:windows}) for this purpose. It turns out that current window types are not sufficient for this purpose as well.
\end{comment}

==> texFiles/extraction.tex <==
%%\newpage

\begin{comment}
\subsection{Non-Primitive Event Detection}
they don't output a relational representation. Therefore, in this work we employ a heuristic-based algorithm (which generates relational representation) designed by ~\cite{DBLP:conf/isvc/AnnappaCA16} for pre-processing. The stream processing framework represented in this work doesn't rely on how efficiently contents are extracted. Therefore any current pre-processing technique can be employed to generate the tuple representations that is needed for this work. We have used both Matlab and OpenCV.

In addition to the above, to answer queries in \textbf{Situations -- Set 2}, some activities (also called events) may have to be detected. This can be done either using IVA techniques or others. Data representation may be difficult as some information may be difficult to retain if IVA techniques are used. We explore and propose streaming processing approach for this by using continuous queries as event generators and compose them. For example, an object moving forward, object turning right or left, overlap of different objects over a short period may be needed for composing higher-level actions or events. We propose to detect some of these events using a combination  of stream and event processing as elaborated in section~\ref{sec:cql-vaimplementation}. 

\end{comment}



%




